OmniSDF: Scene Reconstruction using Omnidirectional Signed Distance Functions and Adaptive Binoctrees

We present a method to reconstruct indoor and outdoor static scene geometry and appearance from an omnidirectional video moving in a small circular sweep. This setting is challenging because of the small baseline and large depth ranges, making it difficult to find ray crossings. To better constrain the optimization, we estimate geometry as a signed distance field within a spherical binoctree data structure and use a complementary efficient tree traversal strategy based on a breadth-first search for sampling. Unlike regular grids or trees, the shape of this structure well-matches the camera setting, creating a better memory-quality trade-off. From an initial depth estimate, the binoctree is adaptively subdivided throughout the optimization; previous methods use a fixed depth that leaves the scene undersampled. In comparison with three neural optimization methods and two non-neural methods, ours shows decreased geometry error on average, especially in a detailed scene, while significantly reducing the required number of voxels to represent such details.

==> sec/finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/intro.tex <==
\section{Introduction}
\label{sec:intro}

3D surface reconstruction from image collections has been a steady goal in computer vision area for its extensive applications for rendering and VR/AR experiences. Recently, the emergence of volumetric rendering pipeline for training nerual implicit functions has dramatically improved the mesh reconstruction quality of objects and unbounded scenes from multi-view images.
State of the art studies has shown expressive power of neural implicit function by reconstructing heritages from internet photo collections~\cite{sun2022neural} and succeeded to capture high fidelity surface details~\cite{li2023neuralangelo} of large-scale scene reconstruction benchmarks~\cite{knapitsch2017tanks}.
However, image-based multi-view geometry reconstructions pipeline always suffers from immense cost in data acquisition steps. Due to the limited field of view that a perspectic camera can capture, we need delecate efforts to calibrate and align tremendeous amounts of images without unseen regions.
As an alternative, our paper adopts omnidirectional video for 3D surface reconsturction of large-scale unbounded scenes.

Panoramic imagings are widely studied for immersive 3D scene understandings due to its ability to capture the scene's omnidirectional enviornments in one shot. Various tasks like spherical depth estimation, semantic understandings for indoor scenes, and novel view synthesis are actively investigated, yet, there is a sole work that tackles large scene 3D surface reconstruction directly from omnidirectional videos. Our work further investigates capturing high-fidelity details of large scene surfaces from omnidirectional video using neural implicit representation. As previous works that aimed at novel view synthesis from omnidirectional videos with neural and non-neural methods~\cite{choi2023balanced, bertel2020omniphotos} did, we follow the setup that captures the scene with a single circular sweep of a 360\degree camera for simplicity of data acquisition setup.

The main challenges of training neural implicit function from omnidirectional video with a narrow baseline come from the innate sparsity of rays crossing the volume under optimization. Concurrent works that focus on neural surface reconstruction assume scenes contents in interest are bounded in a unit cube or sphere and cameras observe in an inward direction from the outside of unit space~\cite{wang2021neus, sun2022neural, li2023neuralangelo} or has a progressive free trajectory~\cite{guo2023streetsurf}. On the other hand, our input image sets observe the scene at the sphere center in outward-facing directions. Therefore, we need a new model to subdivide an unbounded sphere space for efficient training.

Therefore, we propose a novel training model for neural implicit representations in outward-facing sphere space by extending the binoctree data structure~\cite{jang2022egocentric}. Binoctree structure was previously used for subdividing a spherical space without voxel elongation. However, the grid structure was fixed regardless of initial depth accuracy, and TSDF values were fused.
In our work, we first subdivide the space and collect coarse voxels that possibly contain the surface. Using initial coarse voxels as geometry guidance, we adaptively subdivide the voxel during the training. The obtained finer voxels are also used for sampling, therefore effectively narrowing down the sampling regions toward the surface location.
We show that our adaptive space subdivision and sampling policy effectively outstands the results of existing classical and neural surface reconstructions for given omnidirectional video input in both synthetic and real-world domains.




==> sec/preamble.tex <==
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}



==> sec/rebuttal.tex <==
\def\CqHJ{{\color{red}CqHJ}}
\def\qaEi{{\color{darkgreen}qaEi}}
\def\S2Yu{{\color{blue}S2Yu}}


\noindent 
Thank you for your detailed and thoughtful reviews. 

\mparagraph{[\CqHJ,\S2Yu] High-level motivation}
Neural SDF reconstruction is difficult in large unbound scenes. The major challenge is how to overcome the difficulty of training a neural SDF with sparse ray crossings in a 360$\degree$ image set. For large spaces, we might think of applying a contraction function, like in concurrent neural radiance field studies. However, space warping violates the definition of an SDF and invalidates the sphere tracing algorithm [7].
Our contribution improves neural SDF methods by efficiently increasing the sampling rate near surfaces to deal with sparse ray crossings in unbounded scenes.


\mparagraph{[\CqHJ,\S2Yu] Method differences w.r.t.~[8]}
Our work uses the binoctree data structure and preprocessing from [8], but distinguishes itself in the reconstruction algorithm. 
Unlike [8], which directly integrates the SDF from depth maps, our method employs a neural network for SDF definition. 
Additionally, while [8] relies on initial depth maps for a fixed subdivision binoctree, our approach adaptively refines the binoctree during reconstruction. 
This difference allows our method to have continuous SDF input coordinates, with the binoctree only determining sampling for reconstruction. 
As a result, we can adjust the output mesh resolution post-training by resampling the neural network, a process facilitated by integrating spherical binoctrees into a differentiable rendering pipeline with efficient ray intersection and tree-searching modules. This is a novel aspect of our work not possible with existing approaches.



\mparagraph{[\CqHJ,\S2Yu] Quality w.r.t.~[8]}
Challenges in neural reconstruction are different than those in classical methods. 
Given that we claim to improve neural methods, our method does show improvement in comparison to other neural methods like NeuS and Neuralangelo. 
Neural approaches sometimes fail to recover distant surfaces or certain hollow regions that classical [8] does, e.g., supplemental Fig.~4 shows failures of concurrent neural SDF methods like the floor region in \emph{lone-monk}. 
But, neural methods can recover details and smooth surfaces that [8] does not. 
We acknowledge that comparing to [8] is not completely fair, but [8] was the only work we knew that reconstructed a surface mesh for a large outdoor scene from narrow-baseline 360$\degree$ imagery in a memory-efficient way.

\mparagraph{[\CqHJ] Synthetic training data}
We collected 3D scenes from the Blender Online Community and the McGuire Computer Graphics Archive and rendered spherical RGBD video with Blender. The camera has a circular trajectory within a central region inside the architectural scenes. We rendered 200 equirectangular frames at 2048 $\times$ 1024 pixels. We will add examples to the supplement.
\IGNORE{
\begin{figure}[tp]
	\centering
	\includegraphics[width=0.94\linewidth]{figs/synthetic_dataset} 
	\vspace{-4mm}
\caption{\label{fig:synthetic_dataset}
Our synthetic training dataset example.}
	\vspace{-5mm}
\end{figure} 
}

\mparagraph{[\CqHJ] 3D pointcloud coordinates}
We use a global coordinate frame in metric units. This is possible as we input per-frame camera poses and calibrated depth maps. For neural network training, we rescale it: we place the origin at the center of the cameras and scale all surfaces of interest into a unit sphere. The binoctree uses the rescaled coordinates. Please refer to L216 and L322.
We will rephrase and merge this into the preprocessing and binoctree construction section, including the near sphere bound and far sphere bounds so that all preprocessing is explained together.

\mparagraph{[\CqHJ] Omni-depth estimation}
We estimate depth for the initial tree construction using the public-trained model and code from [8].
 We will add this to the preprocessing.



\mparagraph{[\CqHJ] Rendering weight}
We define the rendering weight from the SDF value, following NeuS (described in L228), 
We will add this to Sec.~3. 

\mparagraph{[\CqHJ] Regularize SDF regression}
We use only the losses described in the paper, with no regularization terms. Regularizers can always be added, but hyperparameters are always specific to the data domain and must be tuned to trade smoothness/sharpness. This would be true if we added them to our method too, e.g., like Neuralangelo's Hessian regularizer, but this is orthogonal to our contribution.
\IGNORE{Compared to other losses, Supplemental Table~1 shows that depth guidance with our coarse and fine voxels achieves better results compared to a method that just adds a depth supervision loss.
At the method level, our paper compares to another regularization method via Neuralangelo. This uses the Hessian term to regularize the smoothness of surfaces. Supplemental Table~2 shows our improved quantitative and qualitative depth accuracy over Neuralangelo, but further investigation is necessary as adding such a  regularizer to our method would affect the final result. }

\mparagraph{[\CqHJ] Dynamic partitioning purely relies on SDF}
We investigated the geometry changes before deciding on the subdivision schedule.
For example, Supplemental Figure 5 shows that the geometrical improvement of \emph{Sponza} between 10K and 100K is not distinguishable regardless of loss convergence when the sampling strategy is limited to sphere sampling and coarse voxel sampling. After this observation, we concluded that updating the voxel per 10K steps will not burden the efficiency due to mis-subdivision.

\mparagraph{[\CqHJ] Efficiency}
Our work makes significant memory efficiency gains in its use of space and sampling of space. Compared to neural reconstruction works that use Cartesian voxel grids~\cite{sun2022neural_rebuttal}, for the \emph{Sponza} scene, to subdivide voxel as small as minimum sphoxel size (1.25e-10), the tree height should be at least 11. Considering that the maximum depth of our binoctree was 9, prior work needs an extra $8^{10}+8^{11}$ number of child voxels---more than 36GB extra than ours.

\mparagraph{[\qaEi] Runtime}
To process the \emph{Sponza} scene (Fig.~5) with 200 images, 
COLMAP took 10 hours,
NeuS-Facto took 25 minutes, 
[8] took 30 minutes,
NeuS took 5.5 hours, 
our method took 12.5 hours,
and Neuralangelo took 31 hours.




\mparagraph{[\qaEi] Definitions of $\mathbf{o}$ and $\mathbf{v}$}
$\mathbf{o}$ is the ray origin and $\mathbf{v}$ is the ray direction. We will clarify this in the paper.





\IGNORE{
\mparagraph{[\S2Yu] Separating author contribution from the technical details of [8]}
We give background at the beginning of section 3 (Lines 196- 243): we leverage [8]’s initial spherical binoctree (Lines 205 - 224). 
Other components described after Line 244 in Section 3 (particularly sphoxel intersection in Section 3.1 and sampling strategy and adaptive subdivision in Section 3.2) are our contributions to the method.
We will add a background subsection to further disambiguate our contributions.
}

\mparagraph{[\S2Yu] Figure~4}
We will redraw Fig.~4 to better show that our adaptive approach increases sampling near the surface. 
\IGNORE{
\begin{figure}[h]
	\centering
	\includegraphics[width=0.94\linewidth]{figs/sampling_results_rebittal} 
	\vspace{-5mm}
	\label{fig:sampling_results}
\end{figure} 
}

